The Lyman break analogue Haro 11: spatially resolved chemodynamics with VLT FLAMES

Using VLT/FLAMES optical integral field unit observations, we present the first spatially resolved spectroscopic study of the well known blue compact galaxy Haro11, thought to be a local analogue to high redshift Lyman Break Galaxies. Haro11 displays complex emission line profiles, consisting of narrow (FWHM<200 km/s) and broad (FWHM 200-300 km/s) components. We identify three distinct emission knots kinematically connected to one another. A chemodynamical analysis is presented, revealing that spatially resolved ionic and elemental abundances do not agree with those derived from integrated spectra across the galaxy. We conclude that this is almost certainly due to the surface-brightness-weighting of electron temperature in integrated spectra, leading to higher derived abundances. We find that the eastern knot has a low gas density, but a higher temperature (by ~4,000 K) and consequently an oxygen abundance ~0.4 dex lower than the neighbouring regions. A region of enhanced N/O is found specifically in Knot C, confirming previous studies that found anomalously high N/O ratios in this system. Maps of the Wolf-Rayet feature at 4686A reveal large WR populations (~900-1500 stars) in Knots A and B. The lack of WR stars in Knot C, combined with an age of ~7.4 Myr suggest that a recently completed WR phase may be responsible for the observed N/O excess. Conversely, the absence of N-enriched gas and strong WR emission in Knots A and B suggests we are observing these regions at an epoch where stellar ejecta has yet to cool and mix with the ISM.

==> tables/Avg_abund.tex <==
\begin{table}
\begin{center}
\begin{footnotesize}
\title{Haro~11: Average SFR ionic and elemental abundances derived from maps.}
\begin{tabular}{|l|c|c|c|}
\hline   
 & multicolumn{3}{C1} \\
N$^+/H^+$ & 2.99811e-06 & 5.47288e-06 & 2.57567e-06 \\  
O$^+/H^+$ & 4.00500e-05 & 4.02350e-05 & 9.34432e-05 \\  
O$^{++}/H^+$ & 2.52401e-05 & 5.18536e-05 & 8.27056e-05 \\  
Ne$^{++}/H^+$ & 1.46718e-05 & 3.11601e-05 & 3.47433e-05 \\  
S$^+/H^+$ & 3.21578e-07 & 2.77420e-07 & 1.93593e-07 \\  
O/H & 4.30401e-05 & 8.72604e-05 & 0.000124236 \\  
N/H & 9.83869e-06 & 1.65427e-05 & 3.35404e-05 \\  
Ne/H & 2.48454e-05 & 5.38307e-05 & 5.21427e-05 \\  
S/H & 2.83478e-06 & 1.38940e-06 & 3.22912e-06 \\  
log(N/O) & -NaN & -NaN & -NaN \\  
log(Ne/O) & 0.0498029 & 0.210192 & 0.00000 \\  
log(S/O) & -NaN & -NaN & -NaN \\  
12+log(O/H) & 7.43594 & 7.83272 & 8.04819 \\  
Z/\Zsol & 0.0878370 & 0.178083 & 0.253543 \\  
 & multicolumn{3}{C2} \\
N$^+/H^+$ & 1.64245e-06 & 9.35080e-06 & 0.00000 \\  
O$^+/H^+$ & 2.34900e-05 & 6.44120e-05 & 0.00000 \\  
O$^{++}/H^+$ & 1.44580e-05 & 5.60000e-05 & 0.00000 \\  
Ne$^{++}/H^+$ & 1.18150e-08 & 1.71488e-08 & 0.00000 \\  
S$^+/H^+$ & 8.54400e-08 & 4.45460e-07 & 0.00000 \\  
O/H & 2.03305e-05 & 0.000120412 & 0.00000 \\  
N/H & 4.23151e-06 & 1.76567e-05 & 0.00000 \\  
Ne/H & 1.64996e-08 & 3.66585e-08 & 0.00000 \\  
S/H & 7.14217e-07 & 2.62462e-06 & 0.00000 \\  
log(N/O) & -NaN & -NaN & -NaN \\  
log(Ne/O) & -NaN & -NaN & -NaN \\  
log(S/O) & -NaN & -NaN & -NaN \\  
12+log(O/H) & 7.20352 & 8.00427 & 0.00000 \\  
Z/\Zsol & 0.0414908 & 0.245739 & 0.00000 \\  
\hline
\end{tabular}
\caption{}
\label{tab:haro11_avg_map}
\end{footnotesize}
\end{center}
\end{table}


==> tables/Haro11_SFRegAges.tex <==
\begin{table*}
\begin{center}
\begin{small}
\caption{Age of the latest star formation episode and current star formation rates.}
\begin{tabular}{lccc}

 & Knot A & Knot B & Knot C\\
 \hline
% & \multicolumn{3}{c}{Starburst ages (Myr)}\\
 %\cline{2-4}

%Model &  Knot C & Knot B & Knot A \\
%Padova-AGB PH &        7.71$\pm$       0.85 &        4.81$\pm$       0.10 &        5.26$\pm$       0.19\\
%Padova-AGB LH &        7.66$\pm$       0.88 &        4.71$\pm$       0.10 &        5.11$\pm$       0.16\\
%Geneva-High PH &        7.31$\pm$       0.68 &        4.21$\pm$       0.16 &       4.66$\pm$       0.19\\
%Geneva-High LS &        7.06$\pm$       0.82 &        3.66$\pm$       0.36 &       4.41$\pm$       0.16\\



%& \multicolumn{3}{c}{Star formation rates (M$_\odot$ yr$^{-1}$)}\\
%\cline{2-4}


SFR(H$\alpha$)$^a$(M$_\odot$ yr$^{-1}$)    & 1.87$\pm$0.06           & 4.36$\pm$0.24 & 0.73$\pm$0.03   \\
SFR(H$\alpha$)$^b$ (M$_\odot$ yr$^{-1}$)   & 1.03$\pm$0.03           & 2.40$\pm$0.13 & 0.40$\pm$0.01 \\

%& \multicolumn{3}{c}{$\Sigma$ (M$_\odot$ yr$^{-1}$ kpc$^{-2}$)}\\
\cline{2-4}
$\Sigma$ (M$_\odot$ yr$^{-1}$ kpc$^{-2}$) & 2.64 & 2.14 & 1.02 \\

\hline \label{tab:SFRs}
\end{tabular}
\begin{description}
\item[$^a$] Derived using the relationship between SFR and $L$(H$\alpha$) from
\citet{Kennicutt:1998}.

\item[$^b$] Corrected for sub-solar metallicities following \citet{Bicker:2005}.

\end{description}
\end{small}
\end{center}
\end{table*}


==> tables/UM448_SFRegAges.tex <==
\begin{table*}
\begin{center}
\begin{small}
\caption{Age of the latest star formation episode and current star formation rates.}
\begin{tabular}{lccc}
\hline
 & \multicolumn{3}{c}{Starburst ages (Myr)}\\
 \cline{2-4}
Model &  Knot C & Knot B & Knot A \\
Padova-AGB PH &        7.71$\pm$       0.85 &        4.81$\pm$       0.10 &        5.26$\pm$       0.19\\
Padova-AGB LH &        7.66$\pm$       0.88 &        4.71$\pm$       0.10 &        5.11$\pm$       0.16\\
Geneva-High PH &        7.31$\pm$       0.68 &        4.21$\pm$       0.16 &        4.66$\pm$       0.19\\
Geneva-High LS &        7.06$\pm$       0.82 &        3.66$\pm$       0.36 &        4.41$\pm$       0.16\\
\hline \label{tab:EWs}
\end{tabular}
\end{small}
\end{center}
\end{table*}


==> tables/haro11_abund.tex <==
\begin{landscape}
\begin{table*}

\begin{center}
\begin{footnotesize}
\title{Haro~11: Abundances for summed spectra over individual SF regions}
\begin{tabular}{|l|cc|cc|cc|}
\hline					


		&\multicolumn{2}{c|}{SFR1}								&\multicolumn{2}{c|}{SFR2}								&\multicolumn{2}{c|}{SFR3}							\\
\hline																									
	&	C1			&	C2			&	C1			&	C2			&	C1			&	C2			\\
\hline																									
\elt	&	11,671	$\pm$	747	&	17,947	$\pm$	2,674	&	12,058	$\pm$	886	&	10,864	$\pm$	824	&	12,216	$\pm$	1,075	&	9,627	$\pm$	542	\\
\eld	&	10	$\pm$	50	&	286	$\pm$	182	&	237	$\pm$	121	&	1,265	$\pm$	324	&	166	$\pm$	135	&	218	$\pm$	116	\\
	&				&				&				&				&				&				\\
\op/\hp	&	4.28E-05	$\pm$	1.32E-05	&	2.83E-05	$\pm$	2E-05	&	1.08E-04	$\pm$	3.42E-05	&	8.37E-05	$\pm$	2.43E-05	&	8.26E-05	$\pm$	3.08E-05	&	9.80E-05	$\pm$	2.92E-05	\\
\opp/\hp	&	6.52E-05	$\pm$	1.74E-05	&	1.90E-05	$\pm$	9E-06	&	1.91E-04	$\pm$	5.81E-05	&	3.63E-04	$\pm$	1.59E-05	&	7.82E-05	$\pm$	2.87E-05	&	1.43E-04	$\pm$	4.04E-05	\\
O/H	&	1.08E-04	$\pm$	2.18E-05	&	4.72E-05	$\pm$	2.02E-05	&	2.99E-04	$\pm$	6.74E-05	&	4.47E-04	$\pm$	2.90E-05	&	1.61E-04	$\pm$	4.21E-05	&	2.41E-04	$\pm$	4.98E-05	\\
$12+log(O/H)$	&	8.03	$\pm$	0.09	&	7.67	$\pm$	0.18	&	8.48	$\pm$	0.10	&	8.65	$\pm$	0.03	&	8.21	$\pm$	0.11	&	8.38	$\pm$	0.09	\\
	&				&				&				&				&				&				\\
\np/\hp	&	5.75E-06	$\pm$	1.30E-06	&	2.38E-06	$\pm$	8.83E-07	&	8.05E-06	$\pm$	2.15E-06	&	5.33E-06	$\pm$	1.48E-06	&	1.43E-06	$\pm$	4.70E-07	&	8.04E-06	$\pm$	1.84E-06	\\
ICF(N)	&	2.52	$\pm$	0.93	&	1.67	$\pm$	1.29	&	2.76	$\pm$	1.07	&	5.34	$\pm$	1.59	&	1.95	$\pm$	0.89	&	2.46	$\pm$	1.29	\\
N/H	&	1.45E-05	$\pm$	6.27E-06	&	3.98E-06	$\pm$	3.40E-06	&	2.22E-05	$\pm$	1.05E-05	&	2.84E-05	$\pm$	1.16E-05	&	2.79E-06	$\pm$	1.57E-06	&	1.98E-05	$\pm$	1.37E-05	\\
$[N/O]$	&	-0.87	$\pm$	0.21	&	-1.07	$\pm$	0.41	&	-1.13	$\pm$	0.22	&	-1.20	$\pm$	0.18	&	-1.76	$\pm$	0.27	&	-1.09	$\pm$	0.22	\\
	&				&				&				&				&				&				\\
\nepp/\hp	&	7.05E-06	$\pm$	4.23E-06	&	9.34E-06	$\pm$	5.70E-06	&	1.46E-05	$\pm$	7.53E-06	&	3.05E-05	$\pm$	1.25E-05	&	2.47E-05	$\pm$	1.03E-05	&	4.71E-05	$\pm$	1.51E-05	\\
ICF(Ne)	&	1.66	$\pm$	0.56	&	2.49	$\pm$	2.33	&	1.57	$\pm$	0.85	&	1.23	$\pm$	0.61	&	2.06	$\pm$	1.34	&	1.68	$\pm$	0.76	\\
Ne/H	&	1.17E-05	$\pm$	8.02E-06	&	2.33E-05	$\pm$	2.60E-05	&	2.29E-05	$\pm$	1.71E-05	&	3.76E-05	$\pm$	2.41E-05	&	5.07E-05	$\pm$	3.92E-05	&	7.94E-05	$\pm$	3.18E-05	\\
$[Ne/O]$	&	-0.97	$\pm$	0.31	&	-0.31	$\pm$	0.60	&	-1.12	$\pm$	0.38	&	-1.08	$\pm$	0.33	&	-0.50	$\pm$	0.41	&	-0.48	$\pm$	0.37	\\
	&				&				&				&				&				&				\\
\Sp/\hp	&	5.14E-07	$\pm$	1.30E-07	&	3.66E-07	$\pm$	0E+00	&	6.09E-07	$\pm$	7.62E-07	&	7.26E-07	$\pm$	1.70E-07	&	2.47E-05	$\pm$	1.99E-07	&	5.81E-07	$\pm$	1.33E-07	\\
ICF(S)	&	1.09	$\pm$		&	1.02	$\pm$		&	1.11	$\pm$		&	1.29	$\pm$		&	1.04	$\pm$		&	1.08	$\pm$		\\
S/H	&	3.84E-06	$\pm$		&	2.44E-06	$\pm$		&	4.69E-06	$\pm$		&	7.10E-06	$\pm$		&	1.71E-04	$\pm$		&	4.30E-06	$\pm$		\\
$[S/O]$	&	-1.45	$\pm$		&	-1.29	$\pm$		&	-1.80	$\pm$		&	-1.80	$\pm$		&	0.03	$\pm$		&	-1.75	$\pm$		\\

\hline
\end{tabular}

\caption{Ionic and elemental abundances for Haro~11, derived from summed IFU spectra over each region defined in Fig.~\ref{fig:haro11_SFR}, (corresponding fluxes are listed in Tables~\ref{tab:Haro11-1}--\ref{tab:Haro11-3}).  All ionisation correction factors (ICFs) are taken from \citet{Barlow:1994}.}
\label{tab:haro11_ab}
\end{footnotesize}
\end{center}

\end{table*}
\end{landscape}


==> tables/haro11_avg_abund.tex <==
\begin{table}
\begin{center}
\begin{footnotesize}
\title{Haro~11: Average SFR ionic and elemental abundances derived from maps.}
\begin{tabular}{|l|c|c|c|}
\hline   
 & \multicolumn{3}{c|}{C1} \\
\cline{2-4}
& SFR1 & SFR & SFR 3 \\
\hline   
N$^+/H^+$ &  2.998e-06$\pm$ 1.854e-06 &  5.473e-06$\pm$ 3.476e-06 &  2.576e-06$\pm$ 8.107e-07 \\  
O$^+/H^+$ &  4.005e-05$\pm$ 2.103e-05 &  4.024e-05$\pm$ 3.428e-05 &  4.153e-05$\pm$ 2.935e-05 \\  
O$^{++}/H^+$ &  2.524e-05$\pm$ 1.747e-05 &  5.185e-05$\pm$ 3.640e-05 &  8.271e-05$\pm$ 3.086e-05 \\  
Ne$^{++}/H^+$ &  1.467e-05$\pm$ 1.055e-05 &  3.116e-05$\pm$ 1.569e-05 &  3.474e-05$\pm$ 7.605e-06 \\  
S$^+/H^+$ &  3.216e-07$\pm$ 1.878e-07 &  2.774e-07$\pm$ 2.678e-07 &  1.936e-07$\pm$ 7.401e-08 \\  
O/H &  4.304e-05$\pm$ 4.188e-05 &  8.726e-05$\pm$ 6.027e-05 &  1.242e-04$\pm$ 4.861e-05 \\  
N/H &  9.839e-06$\pm$ 1.276e-06 &  1.654e-05$\pm$ 1.232e-05 &  1.491e-05$\pm$ 1.935e-05 \\  
Ne/H &  2.485e-05$\pm$ 2.555e-05 &  5.383e-05$\pm$ 3.311e-05 &  5.214e-05$\pm$ 1.731e-05 \\  
S/H &      0.000$\pm$     0.000 &      0.000$\pm$     0.000 &      0.000$\pm$     0.000 \\  
log(N/O) &     -0.880$\pm$     0.168 &     -0.812$\pm$     0.354 &     -1.050$\pm$     0.457 \\  
log(Ne/O) &     -0.233$\pm$     0.154 &     -0.167$\pm$     0.182 &     -0.351$\pm$     0.155 \\  
log(S/O) &     -1.436$\pm$     0.185 &     -1.889$\pm$     0.347 &     -1.960$\pm$     0.429 \\  
12+log(O/H) &      7.436$\pm$     0.448 &      7.833$\pm$     0.332 &      8.048$\pm$     0.238 \\  
Z/\Zsol &      0.088$\pm$     0.085 &      0.178$\pm$     0.123 &      0.254$\pm$     0.099 \\  
\hline   
 & \multicolumn{3}{c|}{C2} \\
\cline{2-4}
& SFR1 & SFR & SFR 3 \\
\hline   
N$^+/H^+$ &  1.642e-06$\pm$ 4.925e-07 &  9.351e-06$\pm$ 3.461e-06 &  1.000e+03$\pm$ 0.000e+00 \\  
O$^+/H^+$ &  2.349e-05$\pm$ 9.857e-06 &  6.441e-05$\pm$ 4.175e-05 &  1.000e+03$\pm$ 0.000e+00 \\  
O$^{++}/H^+$ &  1.446e-05$\pm$ 6.035e-06 &  5.600e-05$\pm$ 3.337e-05 &  1.000e+03$\pm$ 0.000e+00 \\  
Ne$^{++}/H^+$ &  1.182e-08$\pm$ 4.400e-09 &  1.715e-08$\pm$ 1.129e-08 &  1.000e+03$\pm$ 0.000e+00 \\  
S$^+/H^+$ &  8.544e-08$\pm$ 8.480e-08 &  4.455e-07$\pm$ 1.791e-07 &  1.000e+03$\pm$ 0.000e+00 \\  
O/H &  2.033e-05$\pm$ 1.694e-05 &  1.204e-04$\pm$ 7.402e-05 &  1.000e+03$\pm$ 0.000e+00 \\  
N/H &  4.232e-06$\pm$ 5.356e-08 &  1.766e-05$\pm$ 6.531e-06 &  1.000e+03$\pm$ 0.000e+00 \\  
Ne/H &  1.650e-08$\pm$ 1.315e-08 &  3.666e-08$\pm$ 2.399e-08 &  1.000e+03$\pm$ 0.000e+00 \\  
S/H &      0.000$\pm$     0.000 &      0.000$\pm$     0.000 &   1000.000$\pm$     0.000 \\  
log(N/O) &     -1.019$\pm$     0.147 &     -0.788$\pm$     0.169 &   1000.000$\pm$     0.000 \\  
log(Ne/O) &     -3.079$\pm$     0.067 &     -3.524$\pm$     0.075 &   1000.000$\pm$     0.000 \\  
log(S/O) &     -2.914$\pm$     1.860 &     -1.615$\pm$     0.134 &   1000.000$\pm$     0.000 \\  
12+log(O/H) &      7.204$\pm$     0.307 &      8.004$\pm$     0.298 &   1000.000$\pm$     0.000 \\  
Z/\Zsol &      0.041$\pm$     0.035 &      0.246$\pm$     0.151 &   1000.000$\pm$     0.000 \\  
\hline
\end{tabular}
\caption{Haro~11: Average SFR ionic and elemental abundances derived from maps.}
\label{tab:haro11_avg_map}
\end{footnotesize}
\end{center}
\end{table}


==> tables/haro11_avg_abund_binnedv1.tex <==
\begin{table*}
\begin{center}
\begin{footnotesize}
%\title{UM~448: Weighted Average SFR ionic and elemental abundances derived from maps.}
\begin{tabular}{|l|c|c|c|c}
\hline   
 & \multicolumn{3}{c|}{C1} & \multicolumn{1}{c|}{C2} \\
\cline{2-5}
& Knot A & Knot B & Knot C & Knot B   \\
\hline   

\elt & 12600$\pm$270 & 12100$\pm$230 & 16600$\pm$480  \\
\eld & 410$\pm$20 & 370$\pm$10 & 150$\pm$15 & --                                                                                                                                						\\
\noalign{\vskip4pt}                                                                                                                                                                         			  
O$^+/H^+$ $\times10^5$ &     5.64$\pm$        0.08 &        10.92$\pm$        0.08 &         3.91$\pm$        0.09     &       --	\\
O$^{++}/H^+$ $\times10^5$ &     6.78$\pm$        0.06 &         6.92$\pm$        0.06 &         2.45$\pm$        0.07     &              15.38$\pm$        0.17  		 	\\   
O/H $\times10^4$ &   1.24$\pm$        0.07 &         1.79$\pm$        0.07 &         0.64$\pm$        0.08      &           -- 	\\
12+log(O/H) &     8.09$\pm$        0.03 &         8.25$\pm$        0.03 &         7.80$\pm$        0.04    &               -- 	\\
Z/\Zsol &     0.24$\pm$        0.02 &         0.35$\pm$        0.03 &         0.12$\pm$        0.01  &                -- 	\\
\noalign{\vskip4pt}                                                                                                                                                                         			  
N$^+/H^+$ $\times10^6$ &    2.19$\pm$        0.05 &         5.74$\pm$        0.05 &         3.00$\pm$        0.06       &        20.28$\pm$        0.13   	\\ 
ICF(N) & 2.20 & 1.63 & 1.63 & --- \\
N/H $\times10^6$ &    4.82$\pm$        0.00 &         9.38$\pm$        0.00 &         4.88$\pm$        0.01      &          -- 	\\
log(N$^+$/O$^+$) &      -1.41$\pm$        0.04 &        -1.28$\pm$        0.04 &        -1.12$\pm$        0.05   &           -- 	\\
\noalign{\vskip4pt}                                                                                                                                                                         			  					
Ne$^{++}/H^+$ $\times10^5$ &        2.62$\pm$        0.07 &         3.93$\pm$        0.07 &         1.36$\pm$        0.08   &       -- 	\\
ICF(Ne) & 1.83 & 2.58 & 2.59 & ---  \\	
Ne/H $\times10^5$ &          4.79$\pm$        0.03 &        10.14$\pm$        0.04 &         3.54$\pm$        0.05  &        -- 	\\
log(Ne$^{2+}$/O$^{2+}$) &           -0.41$\pm$        0.04 &        -0.25$\pm$        0.04 &        -0.25$\pm$        0.05  &    -- 	\\
\noalign{\vskip4pt}                                                                                                                                                                         			  
S$^+/H^+$ $\times10^7$ &          3.37$\pm$        0.04 &         4.64$\pm$        0.04 &         6.36$\pm$        0.05  &       18.47$\pm$        0.12 \\   
ICF(S) & 1.06 & 1.02 & 1.02 & ---  \\
S/H $\times10^7$ &         3.66$\pm$        0.04 &         4.82$\pm$        0.04 &         6.54$\pm$        0.05  &           -- 	\\
log(S$^+$/O$^+$) &       -2.22$\pm$        0.04 &        -2.37$\pm$        0.04 &        -1.79$\pm$        0.04   &           -- 	\\

\hline   

\end{tabular}
\caption{Ionic and elemental abundances for Haro~11, with the corresponding \elt\, and \eld\, used in their derivation.  Columns 1--4 refer to abundances derived from maps, weight-averaged over regions defined in Fig.~\ref{fig:haro11_SFR}.   All ionisation correction factors (ICFs) are taken from \citet{Barlow:1994}.}% Column 5 refers to \elt, \eld\, and abundances derived from spectra integrated over UM~448 (corresponding fluxes are listed in Table~\ref{tab:summed_spec}.
\label{tab:haro11_avg_map}
\end{footnotesize}
\end{center}
\end{table*}


































































